Decentralized Matching in a Probabilistic Environment

We consider a model for repeated stochastic matching where compatibility is probabilistic, is realized the first time agents are matched, and persists in the future. Such a model has applications in the gig economy, kidney exchange, and mentorship matching. We ask whether a $decentralized$ matching process can approximate the optimal online algorithm. In particular, we consider a decentralized $stable$ $matching$ process where agents match with the most compatible partner who does not prefer matching with someone else, and known compatible pairs continue matching in all future rounds. We demonstrate that the above process provides a 0.316-approximation to the optimal online algorithm for matching on general graphs. We also provide a $\frac{1}{7}$-approximation for many-to-one bipartite matching, a $\frac{1}{11}$-approximation for capacitated matching on general graphs, and a $\frac{1}{2k}$-approximation for forming teams of up to $k$ agents. Our results rely on a novel coupling argument that decomposes the successful edges of the optimal online algorithm in terms of their round-by-round comparison with stable matching.

==> 3-approx.tex <==
\subsection{Warm-Up: Greedy-Commit is a $\nicefrac{1}{3}$-approximation to optimum online}

Before presenting a more sophisticated analysis, we first give a short proof that Greedy-Commit gives a $\nicefrac{1}{3}$-approximation to the optimal online algorithm. %It suffices to prove the following theorem. 

\begin{theorem}\label{thm:3-approx} 
The expected reward obtained by Greedy-Commit is at least one third of the expected reward of the optimal online algorithm.
\end{theorem}


% $O_t^+$ denote the set of edges that Opt is exploring for the first time in round $t$, and let $O_t \subseteq O_t^+$ denote the subset of those edges that are realized. Let $O_{\le t}$ denote the total set of realized edges selected by Opt in round $t$. Note that all of these sets are \emph{random} in that they depend on the random realizations of the edges in our graph. When we define these random sets, we can imagine first 
% \my{ You are not using the variables $O_i$ or $O_i^+$ in the proof process. Let's not define variables that are not being used. Also the process of decomposition of edges of Opt according to your 2.31 write-up is recursive. Let's keep the same structure across section (you actually also do it here as well, so maybe you can just drop the prev paragraph)}
% We will define $A_t^+$, $A_t$, and $A_{\le t}$ analogously for Greedy-Commit. Namely, $A_t^+$ denotes the set of new edges selected by Greedy-Commit in round $t$, $A_t \subseteq A_t^+$ denotes the subset of $A_t$ that is realized, and $A_{\le t}$ denotes the total set of realized edges selected by Greedy-Commit in round $t$. For convenience, define $A_{\le 0} := \emptyset$. Note that the structure of the Greedy-Commit algorithm guarantees that $A_{\le t} = A_1 \sqcup A_2 \sqcup \ldots \sqcup A_t$. 

Note that the expected reward of Greedy-Commit is simply $\sum_{t=1}^T \mathbb{E}[A_{\le t}]$ and the expected reward of OPT is $\sum_{t=1}^T \mathbb{E}[O_{\le t}]$. So to prove the above theorem it suffices to show $\mathbb{E}[O_{\le t}] \le 3 \cdot \mathbb{E}[A_{\le t}]$ for all $t$.  



% on the round Opt first discovered them in, and whether or not they can be added to the matching given by $A_{\le t-1}$. This motivates the following definitions. For any $i \in [t]$, split the edges in each $O_i$ into two disjoint categories based on whether they can \emph{augment} the matching given by $A_{\le t-1}$. Formally, define $\Aug(O_i) \subseteq O_i$ to be the set of all $e \in O_i$ such that $A_{\le t-1} \cup \{e \}$ is a matching. All other $e \in O_i$ comprise the set $\Adj(O_i)$; equivalently, $\Adj(O_i)$ it is the set of all $e \in O_i$ such that $e$ shares an endpoint with some edge in $A_{\le t-1}$. 

% As our goal is specifically to bound the size of $O_{\le t}$, we will define $\textsc{Aug}_t(O_i)$ to be those edges in $\textsc{Aug}(O_i)$ which are selected by Opt in round $t$. Similarly define $\textsc{Adj}_t(O_i)$ to be those edges in $\textsc{Adj}(O_i)$ which are selected by Opt in round $t$. 

We prove $\mathbb{E}[O_{\le t}] \le 3 \cdot \mathbb{E}[A_{\le t}]$ via two lemmas. The first, the Domination Lemma, makes use of the fact that in each round $i \leq t$, Greedy-Commit selects the matching to add on to $A_{\le i-1}$ that has the largest expected size.

\begin{lemma}[Domination Lemma]\label{lemma:dominationlemma} Fix a round $t$ and define $\textsc{Aug}_i$ for $1 \leq i \leq t$ as in Equations (\ref{eq:aug1}) and (\ref{eq:aug2}). Then, for all $i \leq t$, $\EE[A_i] \ge \EE[\textsc{Aug}_i]$.
\end{lemma}
\begin{proof}
Fix some $i \le t$. Define $h^A$, the \emph{history} of Greedy-Commit, to be the set of matchings it selects in the first $i-1$ rounds, along with the observed outcomes $\{X_e\}$ of all the edges in these matchings. Note $h^A$ is determined uniquely by the sample graph. So we partition the probability space over sample graphs based on the distinct histories they induce on Greedy-Commit in the first $i-1$ rounds. In particular, for any possible history $h$, let $\mathcal{G}_{h}$ denote the class of all sample graphs $G$ such that $h^A(G) = h$. 
%(i.e. Greedy-Commit has history $h$ when run on $G$ for $i-1$ rounds). 
We use $\EE[ A_i \mid \mathcal{G}_{h} ]$ as a shorthand for the expected size of $A_i$, conditioned on the sample graph being in $\mathcal{G}_{h}$, and use $\PP [\mathcal{G}_{h}]$ for the probability that our sample graph is an element of $\mathcal{G}_{h}$. Note then that 
$$\EE[A_i] = \sum_{h} \EE[A_i \mid \mathcal{G}_{h}] \cdot \PP[\mathcal{G}_{h}]$$ 
and similarly $$\EE[\Aug_i] = \sum_{h} \EE[\Aug_i \mid \mathcal{G}_{h}] \cdot \PP[ \mathcal{G}_{h}].$$
It hence suffices to show that $\EE[\Aug_i \mid \mathcal{G}_{h}] \le \EE[A_i \mid \mathcal{G}_{h}]$ for any history $h$. 

To do so, we analyze $\EE[\Aug_i \mid \mathcal{G}_{h}] $ by partitioning $\mathcal{G}_{h}$ based on the different histories these sample graphs induce on OPT. Specifically, for a fixed history $h'$, let $\mathcal{G}_{h, h'}$ denote all sample graphs that induce a history of $h$ on Greedy-Commit and a history of $h'$ on OPT. Then
 $\EE[\Aug_i \mid \mathcal{G}_{h}] = \sum_{h'} \EE[\Aug_i \mid \mathcal{G}_{h, h'}] \cdot  \PP[\mathcal{G}_{h, h'}], $ 
and therefore, to complete the proof of Lemma \ref{lemma:dominationlemma}, it suffices to show that $$\EE[A_i \mid \mathcal{G}_{h}] \ge \EE[ \Aug_i \mid \mathcal{G}_{h, h'}]$$ for any possible histories $h$, $h'$. The rest of the proof is devoted to this inequality. 


% \my{(leaving this here to think about it more tomorrow: in the capacitated case, $N$ is \textbf{not} even disjoint from \textbf{successful} edges of history $h$.)}

Conditioned on our sample graph being in $\mathcal{G}_{h, h'}$, let $N$ be the \textit{new} edges selected by OPT in round $i$ that can augment the matching $A_{\leq i-1}$. As we mentioned earlier, we can assume that OPT is deterministic. So $N$ is uniquely determined by $h$ and $h'$. Also, by definition $N$ is disjoint from all edges in $h'$ and all successful edges in $h$. 
%, because OPT is selecting the edges in $N$ for the first time. $N$ is also disjoint from all successful edges in $h$, because every successful edge in $h$ is in $A_{\le i-1}$ and $N$ contains edges vertex-disjoint from $A_{\le i-1}$. Thus, $N$ consists only of edges that are either observed to be unsuccessful by $h$, or edge that do not belong to either $h$ or $h'$. 

Let $N_0 \subseteq N$ denote those edges in $N$ that belong to neither $h$ nor $h'$. Because edges are independent, for each edge $e$ outside history $h$ or $h'$, the probability that a random sample graph in $\mathcal{G}_{h, h'}$ includes edge $e$ is exactly $p_e$. Therefore, the expected number of edges in $N$ that are successful is given by $\sum_{e \in N_0} p_e$  as all edges in $N \setminus N_0$ are guaranteed to be unsuccessful. 



%We make a simple structural observation about $\mathcal{G}_{h}$ and $\mathcal{G}_{h, h'}$. Namely,  note that $\mathcal{G}_{h}$ consists of all sample graphs with the exact same ``realization" as $h$ on the edges in that history, with every possible subgraph on the other edges of the input graph. This is because edges not in $h$ cannot affect how Greedy-Commit runs in the first $i-1$ rounds. Hence, choosing a random sample graph conditioned on it being in $\mathcal{G}_{h}$ is equivalent to randomly realizing every edge outside of $h$ with the relevant probability. Similarly, choosing a random sample graph, conditioned on it being in $\mathcal{G}_{h, h'}$ is equivalent to randomly realizing every edge outside of $h$ or $h'$ with the relevant probability. Thus, for each edge $e$ outside history $h$ or $h'$, the probability that a random sample graph in $\mathcal{G}_{h, h'}$ includes edge $e$ is exactly $p_e$.

 
% $\EE[\Aug_i \mid \mathcal{G}_{h^A, h^O}]$ is equal to the sum of the probabilities of edges in $\Aug_i^+$.

Furthermore, observe that the set of edges in $N_0$ can feasibly augment $A_{\leq i-1}$ as every edge in $N_0$ is vertex-disjoint from $A_{\le i-1}$, and the edges in $N_0$ form a matching disjoint from $h$. Hence, Greedy-Commit could select edges in $N_0$ in round $i$. By the definition of the Greedy-Commit algorithm, we have $$ \EE[A_i \mid \mathcal{G}_h] \ge \sum_{e \in N_0} p_e.$$ Additionally, note that conditioned on our sample graph being in $\mathcal{G}_{h, h'}$, $\textsc{Aug}_i$ is guaranteed to be a subset of the successful edges in $N_0$, as edges augmenting $A_{\le t}$ must also augment $A_{\le i-1}$. Therefore, $$\sum_{e \in N_0} p_e \ge \EE[\Aug_i \mid \mathcal{G}_{h, h'}].$$ We conclude $$\EE[A_i \mid \mathcal{G}_h] \ge \EE[\Aug_i \mid \mathcal{G}_{h, h'}]$$ as desired. 
 \end{proof} 
 
 
%Conditioned on the base graph being in $\mathcal{G}_{h^A}$, the set $A_{\le i-1}$ is deterministic, and the set of edges that Greedy-Commit selects in round $i$ is deterministic. Let $E$ be this set of edges. As Greedy-Commit is choosing them for the first-time, and they are all realized independently with the appropriate probability when we sample a random $\hat{G} \in \mathcal{G}_{h^A}$, we have that $$\EE[A_i \mid \mathcal{G}_{h^A}] = \sum_{e \in E} p_e.$$


%We use $\mathcal{H}_i^O$ to denote the \emph{history} of Opt through rounds 1 to $i-1$; $\mathcal{H}_i^O$ specifies in each round which matching was selected, and whether the edges selected in this history were realized or not. For any fixed history $\mathcal{H}_i^O$, there may be multiple base graphs $\hat{G}$ that result in Opt having this history; let's refer to the set of these base graphs by $\mathcal{G}_O(\mathcal{H}_i^O).$ When we condition on $\mathcal{H}_i^O$, what we rigorously mean is that we condition on the base graph $\hat{G}$ being in $\mathcal{G}(\mathcal{H}_i^O)$. Similarly, for any fixed history $\mathcal{H}_i^A$ we let $\mathcal{G}_A(\mathcal{H}_i^A)$ denote the set of base graphs that result in Greedy-Commit having the history $\mathcal{H}_i^A$. 

 %select a random base graph, and run both Opt and Greedy-Commit on it. Let $\Aug_i^+$ be \textit{new} edges selected by Opt in round $i$ that can augment the matching $A_{\leq t}$, so $\Aug_i$ is simply the set of edges in $\Aug_i^+$ that are realized. Note that $A_i^+$ and $\Aug_i^+$ are both matchings that can augment $A_{\le i-1}$, and that Greedy-Commit is choosing a set of edges that augments as much as possible given the information it has. However, because Greedy-Commit and Opt may have very different information available to them after $i-1$ rounds, we have to be careful in our analysis. Notice however that after $i-1$ rounds, any edge that \emph{either} Greedy-Commit or Opt knows to be realized cannot be selected in $\Aug_i^+$, as it must consist only of edges that are new to Opt in round $i$ and not in $A_{\le i-1})$. These edges contribute to $\EE[\Aug_i]$, and to prove the result we will argue that Greedy can include all these edges in its selection in round $i$ (and hence does something at least as good). 

% The idea of the proof is as follows. Fix any history of realizations for the edges selected by Opt and Greedy-Commit among the first $i-1$ rounds. Among the edges in $\Aug_i^+$, each is either unexplored by both or known to be unrealized by Greedy-Commit (any edge that Greedy-Commit knows is realized is included in $A_{\le i-1}$). Hence the only edges contributing to the expectation of $\Aug_i$ are unexplored by both Greedy-Commit and Opt. They form a matching that can augment $A_{\le i-1}$; and hence could be selected by Greedy-Commit. But by the optimality 


% Note $\Aug_i$ consists of edges that Opt first learned about in round $i$ which can be added to $A_{\le t}$ (and hence can be added to $A_{\le i-1}$). In round $i$, Opt had no information about these edges, and couldn't be doing anything better than what Greedy-Commit did in round $i$, where it tried to augment $A_{\le i-1}$ as much as possible. This is true even if we give Opt the additional information that Greedy-Commit had after $i-1$ rounds.

%Let $\mathcal{H}^A_i$ denote the history for Greedy-Commit up until but not including round $i$; formally $\mathcal{H}^A_i$ specifies, for each edge selected by Greedy-Commit in in the first $i-1$ rounds, whether the edge was realized or not. Similarly, let $\mathcal{H}^O_i$ denote the history for Opt up until but not including round $i$; formally $\mathcal{H}^O_i$ specifies, for each edge selected by Opt in the first $i-1$ rounds whether the edge was realized or not. Let $\mathcal{H}_i$ denote the combined history of both Greedy-Commit and Opt in the first $i-1$ rounds. 

% We will show $$\EE[A_i \mid \mathcal{H}_i] \ge \EE[\Aug_i \mid \mathcal{H}_i].$$ Note that $A_i^+$ is entirely disjoint from all the edges in $\mathcal{H}^A_i$, but it may include some edges in $\mathcal{H}_i^O$. We hence can partition $A_i^+$ into three sets $X$, $Y$, $Z$ (TODO: better notation) where $Y \subseteq A_i^+$ denotes those edges in $\mathcal{H}_i^O$ that were realized, $Z \subseteq A_i^+$ denotes those edges in $\mathcal{H}_i^O$ that were not realized, and $X \subseteq A_i^+$ denotes those edges in not in $\mathcal{H}_i^O$. With this notation in place, we have that $$ \EE[A_i \mid \mathcal{H}_i ] = |Y| + \sum_{e \in X} p_e.$$

% We will show $$\EE[A_i \mid \mathcal{H}_i^A] \ge \EE[\Aug_i \mid \mathcal{H}_i^O].$$ Note that $A_i^+$ is entirely disjoint from all the edges in $\mathcal{H}^A_i$; hence, $$\EE[A_i \mid \mathcal{H}_i^A] = \sum_{e \in A_i^+} p_e. $$ Note also that $\Aug_i^+$ is entirely disjoint from $\mathcal{H}_i^O$ so $$\EE[\Aug_i \mid \mathcal{H}_i^O] = \sum_{e \in \Aug_i^+} p_e.$$

% but it may include some edges in $\mathcal{H}_i^O$. Let $D \subseteq A_i^+$ denote those edges not in $\mathcal{H}_i^O$ (and hence not in $\mathcal{H}_i$). Clearly $$ \EE[A_i \mid \mathcal{H}_i ] \ge \sum_{e \in D} p_e.$$ Note that this is truly an inequality, as $A_i^+$ may also include edges that are guaranteed to be realized when conditioning on $\mathcal{H}_i^O$. 


%We will show $$\EE[A_i \mid \mathcal{H}_i] \ge \EE[\Aug_i \mid \mathcal{H}_i].$$ Note that $A_i^+$ is entirely disjoint from all the edges in $\mathcal{H}^A_i$, but it may include some edges in $\mathcal{H}_i^O$. Let $D \subseteq A_i^+$ denote those edges not in $\mathcal{H}_i^O$ (and hence not in $\mathcal{H}_i$). Clearly $$ \EE[A_i \mid \mathcal{H}_i ] \ge \sum_{e \in D} p_e.$$ Note that this is truly an inequality, as $A_i^+$ may also include edges that are guaranteed to be realized when conditioning on $\mathcal{H}_i^O$. 

%We now analyze $\EE[\Aug_i \mid \mathcal{H}_i]$. Because $\Aug_i^+$ only includes edges that Opt is exploring for the first time in round $i$, it is clearly disjoint from everything in $\mathcal{H}_i^O$. Note that every edge in $\Aug_i^+$ is clearly not in the realized edges $A_{\le i-1}$, and hence $\Aug_i^+$ is disjoint from the realized edges in $\mathcal{H}_i^A$; it may include unsuccessful edges in $\mathcal{H}_i^A$. Let $D' \subseteq \Aug_i^+$ consist of those edges in $\Aug_i^+$ disjoint from $\mathcal{H}_i^A$ (and hence disjoint from $\mathcal{H}_i$). Note then that $$ \EE[A_i \mid \mathcal{H}_i ] = \sum_{e \in D'} p_e.$$

%The key claim is that $$\sum_{e \in D} p_e \ge \sum_{e \in D'} p_e .$$ This is where we use the optimality of greedy; if we had $\sum_{e \in D} p_e < \sum_{e \in D'} p_e$, consider changing $A_i^+$ by replacing $D$ with $D'$. We just need to check that $D'$ is a matching (which is clearly is) and that $D'$ is disjoint from both $\mathcal{H}_i^A$ and $\mathcal{H}_i^O$ (which it is by definition), so it can be added to $A_i^+ \setminus D$. Hence, if we changed $A_i^+$ by replacing $D$ with $D'$, we would be doing better in expectation which contradicts the optimality of greedy. Hence, we have shown that $$\EE[A_i \mid \mathcal{H}_i] \ge \EE[\Aug_i \mid \mathcal{H}_i].$$ As this holds for any history along the first $i-1$ rounds, taking a weighted average shows $\EE[A_i] \ge \EE[\Aug_i]$ as desired. 

Now, using the Domination Lemma, we can bound 
\begin{align*}
\EE[O_{\le t}] &= \sum_{i=1}^t \Big( \EE[\Aug_i] + \EE[\Adj_i] \Big) 
\le \sum_{i=1}^t \EE[A_i] + \sum_{i=1}^t \EE[\textsc{Adj}_i] 
= \EE[A_{\le t}] +  \sum_{i=1}^t \EE[\textsc{Adj}_i],
\end{align*}
which motivates bounding $\sum_{i=1}^t \EE[\textsc{Adj}_i]$. We do so via a Charging Lemma, related to the fact that two maximal matchings in a graph always have sizes within a factor of 2. 

\begin{lemma}[Charging Lemma]
\label{lemma:charging1}We have $$2 \cdot \EE[A_{\le t}] \ge \sum_{i=1}^t \EE[\textsc{Adj}_i].$$
\end{lemma} 
\begin{proof} Fix a sample graph. Consider any edge $e \in \cup_i \textsc{Adj}_i$. By definition, it is incident to at least one edge in $A_{\le t}$; charge $e$ to one of the edges in $A_{\le t}$ it is incident to. Note that because $\cup_t \textsc{Adj}_t$ forms a matching, every edge in $A_{\le t}$ is charged at most twice. The result follows after averaging over all sample graphs.\end{proof} 

From the Domination Lemma and Charging Lemma, we directly conclude that 
\begin{align*}
\EE[O_{\le t}] &\le \EE[A_{\le t}] + 2\EE[A_{\le t}] \le 3 \EE[A_{\le t}]
\end{align*}
which proves Theorem~\ref{thm:3-approx}. 

==> 5-Enhanced_2.15_approx.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% New Section, 2.15 Approx, Opt Commit %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{2.15 Approx (Greedy Commit VS Opt Commit, Cumulative Reward)}
In the following, we introduce a linear program $(P)$ in which the objective function of $(P)$ guarantees an upper bound on the approximation factor of Greedy Commit Alg, Comparing to Opt Commit, in a cumulative rewards model. Let the variables in $(P)$ be denoted by $X$ and $Y$, where $X$ corresponds to the expected values of sets of edges picked by Alg, and $Y$ corresponds to the expected values of sets of edges picked by Opt  (i.e. $X_{i,j}$ is the variable associated with $O_{i,j}$ and $X_{i,Dis}$ is the variable associated with $O_{i,Dis}$). All these values will be normalized by the expected value $\sum_{t=1}^T \mathbb{E}[|A_{\leq t}|]$, which is the cumulative reward acquired by Alg.

\setcounter{equation}{0}
\begin{align}
\max\;\;\;\;\;\; \sum_{t = 1}^{T}\sum_{i = 1}^{t} \Big( X_{i,Dis} +   \sum_{j = 1}^{T} & X_{i,j} \Big) \hfill  & (Primal)   \\
\text{s.t. \;\;\;\;\;\;\;}
X_{i,Dis} + \sum_{q = j}^{T} X_{i,q} &\leq Y_j \;\; &\forall i,j \in \left \{ 1,2,\cdots, T \right \} \\
\sum_{i = 1}^{T} X_{i,j} &\leq 2 Y_j \;\; &\forall j \in \left \{ 1,2,\cdots, T \right \} \\
\sum_{t = T}^{t} \sum_{i = 1}^{t} Y_{i}  &= \sum_{t = 1}^{T} (T-t+1) Y_{t} \leq 1 \;\; &\\
 Y_i \geq 0, \;  X_{i,Dis} &\geq 0, \;  X_{i,j} \geq 0  \;\; &\forall i,j \in \left \{ 1,2,\cdots, T \right \} 
\end{align}

\noindent Given any solution for Greedy Commit and Opt Commit, we can construct a feasible solution to $(P)$ by setting:
$$X_{i,Dis} = \frac{\mathbb{E}[|\NewOptSucc{i,Dis}|]}{ \sum_{t=1}^T \mathbb{E}[| \RoundAlgSucc{t}|]}, X_{i,j} = \frac{\mathbb{E}[|\NewOptSucc{i,j}|]}{ \sum_{t=1}^T \mathbb{E}[|\RoundAlgSucc{t}|]}, Y_j = \frac{\mathbb{E}[|\NewAlgSucc{j}|]}{\sum_{t=1}^T \mathbb{E}[|\RoundAlgSucc{t}|]}$$
In other words, any solutions for Greedy Commit and Opt Commit must satisfy the inequalities in $(P)$. The objective of $(P)$ in line (1) illustrates the sum of variables associated with successful realizations by Optimum Commit algorithm in rounds $1, \cdots T$. Constraints (2) and (3) follow from corollary \ref{corr:Greedy_Optimality} and lemma \ref{generalized_Charging} respectively, and constraint (4) guarantees that the objective function is more than or equal to the approximation factor for Greedy Commit Algorithm.

\noindent The dual of $(P)$ is:

\setcounter{equation}{0}
\begin{align}
\min\;\;\;\;\;\;  u \hfill  && (Dual) \\
\text{s.t. \;\;\;\;\;\;\;}
\sum_{q = 1}^{j} F_{i,q} + c_j &\geq (T-i+1) \;\; &\forall i,j \in \left \{ 1,2,\cdots, T \right \} \\
\sum_{i = 1}^{T} F_{i,j} + 2c_j &\leq (T-j+1)\times u \;\; &\forall j \in \left \{ 1,2,\cdots, T \right \} \\
\sum_{j = 1}^{T} F_{i,j} &\geq (T-i+1) \;\; &\forall i \in \left \{ 1,2,\cdots, T \right \} \\
 u \geq 0, \; c_{j} \geq 0, \; & F_{i,j} \geq 0  \;\; &\forall i,j \in \left \{ 1,2,\cdots, T \right \} 
\end{align}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% New Section, 2.15 Approx, Opt, not commit%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{2.15 Approx (Greedy Commit VS Opt, Cumulative Reward)}
In the following, we introduce a linear program $(P)$ in which the objective function of $(P)$ guarantees an upper bound on the approximation factor of Greedy Commit Alg, Comparing to Opt, in a cumulative rewards model. Let the variables in $(P)$ be denoted by $X$ and $Y$, where $X$ corresponds to the expected values of sets of edges picked by Alg, and $Y$ corresponds to the expected values of sets of edges picked by Opt (i.e. $X^t_{i,j}$ is the variable associated with $O^t_{i,j}$ and $X^t_{i,Dis}$ is the variable associated with $O^t_{i,Dis}$). All these values will be normalized by the expected value $\sum_{t=1}^T \mathbb{E}[|A_{\leq t}|]$, which is the cumulative reward acquired by Alg.

\setcounter{equation}{0}
\begin{align}
\max\;\;\;\;\;\; \sum_{t = 1}^{T}\sum_{i = 1}^{t} \Big( X^t_{i,Dis} +   \sum_{j = 1}^{T} & X^t_{i,j} \Big) \hfill  & (Primal)   \\
\text{s.t. \;\;\;\;\;\;\;}
X_{i,Dis} + \sum_{q = j}^{T} X_{i,q} &\leq Y_j \;\; &\forall i,j \in \left \{ 1,2,\cdots, T \right \} \\
\sum_{i = 1}^{t} X^t_{i,j} &\leq 2 Y_j \;\; &\forall t, j \in \left \{ 1,2,\cdots, T \right \} \\
\sum_{t = T}^{t} \sum_{i = 1}^{t} Y_{i}  &= \sum_{t = 1}^{T} (T-t+1) Y_{t} \leq 1 \;\; &\\
X^t_{i,j} &\leq X_{i,j} \;\; &\forall t, j \in \left \{ 1,2,\cdots, T \right \}, i \in \left \{ 1,2,\cdots, t \right \} \\
X^t_{i,Dis} &\leq X_{i,Dis} \;\; &\forall t \in \left \{ 1,2,\cdots, T \right \}, i \in \left \{ 1,2,\cdots, t \right \} \\
 Y_i \geq 0, \;  X_{i,Dis} &\geq 0, \;  X_{i,j} \geq 0  & \\
X^t_{i,Dis} \geq 0,& \;  X^t_{i,j} \geq 0  \;\; &\forall i,j,t \in \left \{ 1,2,\cdots, T \right \} 
\end{align}

\noindent Given any solution for Greedy Commit and Opt, we can construct a feasible solution to $(P)$ by setting:
$$X_{i,Dis} = \frac{\mathbb{E}[|\NewOptSucc{i,Dis}|]}{\sum_{i=1}^T \mathbb{E}[|\NewAlgSucc{i}|]}, X_{i,j} = \frac{\mathbb{E}[|\OldOptSucc{i,j}{t}|]}{\sum_{i=1}^T \mathbb{E}[|\NewAlgSucc{i}|]}, Y_i = \frac{\mathbb{E}[|\NewAlgSucc{i}|]}{\sum_{i=1}^T \mathbb{E}[|\NewAlgSucc{i}|]}$$
In other words, any solutions for Greedy Commit and Opt must satisfy the inequalities in $(P)$. The objective of $(P)$ in line (1) illustrates the sum of variables associated with successful realizations by Optimum algorithm in round $1, \cdots , T$. Constraints (2) and (3) follow from corollary \ref{corr:Greedy_Optimality} and lemma \ref{generalized_Charging} respectively, and constraint (4) guarantees that the objective function is more than or equal to the approximation factor for Greedy Commit Algorithm.

\noindent The dual of $(P)$ is:

\setcounter{equation}{0}
\begin{align}
\min\;\;\;\;\;\;  u \hfill  && (Dual) \\
\text{s.t. \;\;\;\;\;\;\;}
\sum_{q = 1}^{j} F_{i,q} - \sum_{t = i}^{T} G^t_{i,j} &\geq 0 \;\; &\forall i,j \in \left \{ 1,2,\cdots, T \right \} \\
C^t_{j} + G^t_{i,j} &\geq 1 \;\; &\forall t,j \in \left \{ 1,2,\cdots, T \right \}, i \in \left \{ 1,2,\cdots, t \right \} \\
\sum_{i = 1}^{T} F_{i,j} + \sum_{t= 1}^{T} 2c^t_j &\leq (T-j+1)\times u \;\; &\forall j \in \left \{ 1,2,\cdots, t \right \} \\
\sum_{j = 1}^{T} F_{i,j} &\geq \sum_{t = i}^{T}G^t_{i,Dis} \;\; &\forall i \in \left \{ 1,2,\cdots, T \right \} \\
G^t_{i,Dis} &\geq 1 \;\; &\forall t \in \left \{ 1,2,\cdots, T \right \}, i \in \left \{ 1,2,\cdots, T \right \} \\
u \geq 0, \; c^t_{j} & \geq 0, \;  F_{i,j} \geq 0  \;\; &\\
G^t_{i,Dis} &\geq 0, \;  G^t_{i,j} \geq 0  \;\; &\forall i,j,t \in \left \{ 1,2,\cdots, T \right \} 
\end{align}

